Dynamically inflated wind models of classical Wolf-Rayet stars

Vigorous mass loss in the classical Wolf-Rayet (WR) phase is important for the late evolution and final fate of massive stars. We develop spherically symmetric time-dependent and steady-state hydrodynamical models of the radiation-driven wind outflows and associated mass loss from classical WR stars. The simulations are based on combining the opacities typically used in static stellar structure and evolution models with a simple parametrised form for the enhanced line-opacity expected within a supersonic outflow. Our simulations reveal high mass-loss rates initiated in deep and hot optically thick layers around T\approx 200kK. The resulting velocity structure is non-monotonic and can be separated into three phases: i) an initial acceleration to supersonic speeds ii) stagnation and even deceleration, and iii) an outer region of rapid re-acceleration. The characteristic structures seen in converged steady-state simulations agree well with the outflow properties of our time-dependent models. By directly comparing our dynamic simulations to corresponding hydrostatic models, we demonstrate explicitly that the need to invoke extra energy transport in convectively inefficient regions of stellar structure and evolution models is merely an artefact of enforcing a hydrostatic outer boundary. Moreover, the "dynamically inflated" inner regions of our simulations provide a natural explanation for the often-found mismatch between predicted hydrostatic WR radii and those inferred from spectroscopy. Finally, we contrast our simulations with alternative recent WR wind models based on co-moving frame radiative transfer for computing the radiation force. Since CMF transfer currently cannot handle non-monotonic velocity fields, the characteristic deceleration regions found here are avoided in such simulations by invoking an ad-hoc very high degree of clumping.

==> comments_Puls.tex <==
% Below Eq 10: solar plasma mixture with completely ionized H and He.

Below: It is commonly believed ...: I'm not sure whether this is
really commonly believed ...

end of Sect. 3.2: You might have a look into WR models by W-R or John H., to check what is the floor value in WRs


Eq. 15: Maybe I'm too silly, but I don't see (without some calculations)
how this Eq. can be derived. And: Is the W on the rhs really the W
from (14), i.e., a constant? In any case, since w(r) changes sign at
vesc, whereas the rhs does not change sign, there is something rotten
\luka{need to redo computation}

% Fig. 1: maybe an indication at the coding-table (right) that this refers to Gamma.

% When you discuss this figure, you might tell that this figure also
% shows that Pg does not play a role in the lower wind, compared to Prad.

% page 3, 2nd §: ... Clearly, this temperature difference ...
% There is some text missing, because you have not mentioned a temp. diff.
% before.

% Eq. 17 and 18.

% Use abs (dv/dr), and tell the people that for negative dv/dr, this is
% only an approximation, since for nonmonotonic flows there is a certain
% coupling of the corresponding resonance zones with similar n*v.


inside Sect. 3.4

(i) give examples for r1 and r2
(ii) argue about decreasing alpha as discussed via phone, i.e,
both ionization effects closing the gaps, and ML effects. 
Moreover, you can tell that it's sort of reassuring that with prototypical alpha you cannot drive the wind to infinity, consistent with earlier findings.

% End of 3.4: see also Fig. 14 in Pauldrach 1993 (SSRv66)


Fig. 3: maybe you already here indicate the location of Rphot.
Personally, here, and in Figs. 6 and 7, I would not use two line-styles,
but indicate the location of Rphot by a short vertical line.
\luka{It is a good suggestion ill make new plots}

Fig. 4: at least from this figure, and even accounting for the
compressed scale, it seems that v(r) is still increasing at your
outermost computational domain. 
\luka{it is scale effect}


Fig. 5 and text: Which physics determines the location of the
sudden increase in grad?



Fig. 6: I guess I'm blind, but in my opinion the switch from solid to
dotted is located below tau=2/3. Please check.
\luka{It is $\tau(R_c)$ plotted there, therefore it is not 2/3}

% Below Eq. 19: as defined here, dtau is not a differential, but just
% part of a differential.

Fig. 10 and or following:

Do you have a specific reason why you haven't directly compared with the
steady-state solution? I know, the time-dependent one goes a bit deeper, but
from what I see, the differences are quite small, and this should be
shown ...

Sect. 4.3

"vinf primarily controlled by the wind conditions": However, since there
is only one luminosity to exploit, I would guess that also Mdot has an
influence, even more if you initiate this quantity by a separate
process (OPAL opacities). I would expect (as also shown in one of the
tables), that if you increase Mdot for a given luminosity, then vinf
should decrease ...


Below Tab. 2
"a high Mdot by exceeding the sonic point" ... I guess, this needs to
be reformulated

last sentence of 4.3.2: I guess you mean that these tests are
explained in the next section. If so, please tell this. Otherwise, 
maybe a couple of more words.

% Eq. 23 and 25: P -> P_g

% Eq. 26: I'm not completely sure whether Eq. 26 is just the normal outer boundary condition, or involves Eq. 25. 

% Before Eq. 28: from your outer boundary, taur=4/3 always, you might argue that your diffusive limit for Prad is justified for the complete static atmosphere, until Rmax (indeed, before coming to this point, I was concerned that this might be a problem).

below: Rphot "is extremely sensitive on Gamma_e"...
Is there a simple reason for this?

% Fig. 12, end of caption: "stellar photospheric Teff" 
% Maybe replace by "hydrostatic Teff", as introduced before?


End of 5.1:

If I understand this correctly: Without MLT++, one would have an enormous inflation, whereas with dynamic inflation, this is "only" a factor of three. Correct? Anyhow, I would guess that even with such an inflation, the time-step issue would still be present.

Sect. 5.2

As earlier discussed: if Rphot would be really at such high v(r), I would speculate that the (optical) profile shapes would be different (shell profiles). Maybe you calculate simple recombination profiles ...

page 10, right, last §: If I remember correctly, the Geneva code prohibits density inversions. This is also a way to prohibit inflation...

Fig. 14: that in a HRD Teff goes "in reversed direction", should be known by any astronomer ...

page 11, 1st §: Maybe as a footnote, please mention which fcl had been assumed for the provided Mdot. (in particular, since later on you discuss clumping). 
